Solving Unique Games over Globally Hypercontractive Graphs

We study the complexity of affine Unique-Games (UG) over globally hypercontractive graphs, which are graphs that are not small set expanders but admit a useful and succinct characterization of all small sets that violate the small-set expansion property. This class of graphs includes the Johnson and Grassmann graphs, which have played a pivotal role in recent PCP constructions for UG, and their generalizations via high-dimensional expanders. Our algorithm shows how to round "low-entropy" solutions to sum-of-squares (SoS) semidefinite programs, broadly extending the algorithmic framework of [BBKSS'21]. We give a new rounding scheme for SoS, which eliminates global correlations in a given pseudodistribution so that it retains various good properties even after conditioning. Getting structural control over a pseudodistribution after conditioning is a fundamental challenge in many SoS based algorithms. Due to these challenges, [BBKSS] were not able to establish strong algorithms for globally hypercontractive graphs, and could only do so for certifiable small-set expanders. Our results improve upon the results of [BBKSS] in various aspects: we are able to deal with instances with arbitrarily small (but constant) completeness, and most importantly, their algorithm gets a soundness guarantee that degrades with other parameters of the graph (which in all PCP constructions grow with the alphabet size), whereas our doesn't. Our result suggests that UG is easy on globally hypercontractive graphs, and therefore highlights the importance of graphs that lack such a characterization in the context of PCP reductions for UG.

==> extra.tex <==
\subsubsection{Bounding the shift potential in certifiable SSE graphs}\label{sec:shift-pot}
\mitali{remove these sections, use only for calculations}

In this section, we will use that in a small-set expander, when the expansion of the approximate partition defined the $f_s$ is low and the objectives $\val(X),\val(X')$ are high, then the shift-partition potential $\Phi(X,X')$ (which is a proxy for the size of the partition parts) is large. 
Further, we will show that this fact has an SOS proof when the graph has an SOS certificate of expansion. 

\mitali{lem:sp-pseudo - restate?}

\begin{proof}[Proof of Lemma~\ref{lem:sp-pseudo}]
Given assignments $(X,X')$ consider the approximate partition defined by the $\{f_s\}_{s \in \Sigma}$ as in (\ref{eq:fs}) and identify $f_s$ with an approximate component $C_s$.
We note that the $f_s$ are close to indicator functions, as they are the product of an indicator and an approximate indicator $p$.
As noted after equation (\ref{eq:fs}), $\Phi_{\beta,\nu}(X,X') = \sum_s \E_{u \sim \pi}[f_s(u)]^2$.
Further, our axioms easily imply that $f_s$ are bounded functions,

\begin{claim}\label{claim:bounded}
From our Unique Games axioms and the axiom that $p \in P_{\beta,\nu}$, we may conclude that the $f_s$ are bounded:
\[
\A_G \cup \{p \in P_{\beta,\nu}\} \vdash_{\tilde{O}(1/\nu)} \{0\le f_s(v) \le 1\}_{s \in \Sigma,v\in V}.
\]
\end{claim}

We provide the proof below in Section~\ref{sec:claim-pfs}.
Thus, we may apply the SSE certificate $\SSE_{\alpha,\gamma}(G)$ guaranteed by the condition of the lemma to all the functions $f_s$ and sum up the equality over $s \in \Sigma$. 
This gives us,
\begin{equation*}
\sum_s \ip{f_s, L f_s}_{\pi} \ge \alpha \sum_s \E_\pi[f_s] + c \left(\gamma \sum_s \E_\pi[f_s] - \sum_s \E_\pi[f_s]^2 \right) - \left(\sum_s 2B_1(f_s) + \sum_s B_2(f_s)  \right).
\end{equation*}
For $B_1(f) = \E_\pi[f - f^{\circ 2}]$ and $B_2(f) = \ip{f - f^{\circ 3}, P f}_\pi$, and $c \ge 0$.
Substituting $\sum_{s} \E_\pi[ f_s]^2 = \Phi_{\beta,\nu}(X,X')$ and re-arranging the expression,
\begin{equation}\label{eq:partition}
\Phi_{\beta,\nu}(X,X') \ge \gamma \sum_s \E_\pi[f_s] + \frac{1}{c}\left(\alpha \sum_s \E_\pi[f_s]  - \left(\sum_s 2B_1(f_s) + \sum_s B_2(f_s)  \right)- \sum_s \ip{f_s, L f_s}_{\pi}\right) .
\end{equation}
We now bound and simplify the remaining terms.
Our goal will be to obtain as large as possible a quantity on the right-hand side.

First, we would like a lower bound on $\sum_{s \in \Sigma} \E_\pi[f_s]$, which measures the total number of vertices included in the approximate partition.
If we were working with the pure shift partition $\Ind[X_u = X_u' + s]$, then this quantity would be $1$; since we have dropped vertices of low objective value, we must prove that we did not remove too many.
\begin{claim}\label{claim:cover}
Under the axioms guaranteed by our lemma, the total number of vertices participating in the approximate partition $\{f_s\}_{s \in \Sigma}$ is large,
$$\A_G \cup \{p \in P_{\beta,\nu}\} \,\, \vdash_{\tilde{O}(1/\nu)} \,\,
    \sum_s \E_\pi[f_s] \geq 1 - \frac{\viol(X)}{1 - \beta - \nu} - \nu.
$$
\end{claim}
This claim follows easily from an averaging argument if we replace $p(x)$ with $\Ind[x \ge \beta]$, since this amounts to removing vertices with at least $ 1-\beta$ incident violated edges in $X$. 
Below, we will show that this claim still holds as an SoS inequality when we use the $\eta$-approximate indicator $p$. 
See Section~\ref{sec:claim-pfs}.

Second, we must argue that the total expansion of the approximate partition is not too large.
The following claim shows that the expansion is bounded by the total violations of $X$ and $X'$:
\begin{claim}\label{claim:expans}
Under the axioms guaranteed by our lemma, the total expansion of the partition is bounded as a function of the total violations in $X$ and $X'$:
$$\A_G \cup \{p \in P_{\beta,\nu}\} \,\, \vdash_{\tilde{O}(1/\nu)} \,\,
    \sum_s \ip{f_s,Lf_s}_\pi \leq \viol(X)+\viol(X') + 2\left(\frac{\viol(X)}{1 - \beta - \nu}\right) + 2\nu.$$
\end{claim}

The proof of this claim uses the fact that in any satisfying assignment for an edge $(u,v)$, $X_u = X_v + s$ for a fixed $s \in \Sigma$, and therefore an edge that crosses the shift partition must be violated in either $X$ or $X'$ since the endpoints differ by a different shift in each assignment.
To account for vertices dropped because their violations are $\ge 1-\beta$, we again use an averaging argument.
We will prove this formally below.

Finally, if the $f_s$ were $0/1$-valued functions, $B_1(f_s)$ and $B_2(f_s)$ would have value $0$.
Since $f_s$ are instead approximately $0/1$ valued, we must show that $B_1(f_s)$ and $B_2(f_s)$ are close to $0$:


\begin{claim}\label{claim:B1}
Under the axioms of our lemma, the $B_1(f_s)$ are small,
$$\A_G \cup \{p \in P_{\beta,\nu}\} \,\, \vdash_{\tilde{O}(1/\nu)} \,\,
\sum_s \E_\pi[f_s - f_s^{\circ 2}] \leq \frac{\viol(X)}{1 - \beta - \nu} + \nu.$$
\end{claim}
\begin{claim}\label{claim:B2}
Under the axioms of our lemma, for any $\eta \in \R_+$ and $\nu < \frac{1}{3}(1-\beta)$, the $B_2(f_s)$ may be bounded by
$$\A_G \cup \{p \in P_{\beta,\nu}\} \,\, \vdash_{\tilde{O}(1/\nu)} \,\,
    \sum_s \ip{f_s - f_s^{\circ 3}, P f_s}_\pi \leq \frac{1}{2\eta} + \eta\left(\frac{\viol(X)}{1 - \beta - \nu} + \nu\right).$$
\end{claim}

When we combine these claims with equation~(\ref{eq:partition}) and simplify, we have the desired inequality, where the parenthesized right-hand side term becomes $K_{\beta,\nu}^{\alpha,\eta}$.
We prove our claims below in Section~\ref{sec:claim-pfs}
\end{proof}

\subsubsection{Proofs of Claims}\label{sec:claim-pfs}
\mitali{skip this section. Have approximate Markov, averaging argument, union bound in prelims, along with approximating indicators.}

We now prove the outstanding claims.
We first record some consequences of our unique games axioms $\A_G$, which will be useful to us:
\begin{fact}\label{fact:ug-axioms}
The unique games constraints $\A_G$ imply the following bounds:
\begin{enumerate}
    \item The local values and violations of variables are in $[0,1]$: $\A_G \vdash_2 \{0 \le \val_u(X) \le 1\} \cup \{0 \le \viol(X) \le 1\}$
    \item The variables $\{\Ind[X_u - X_u' = s]\}_{s\in\Sigma,u \in V(G)}$ satisfy Booleanity and partition constraints,
    \[
    \A_G \vdash_4 \{\Ind[X_u-X_u' = s]^2 = \Ind[X_u - X_u' = s]\}_{u \in V(G), s \in \Sigma} \cup \{\sum_{s \in \Sigma}\Ind[X_u - X_u' = s] = 1\} 
    \]
    \item The partition crossing edges are bounded by the sum of violations:
    \[
    \A_G \vdash_8 \E_{(u,v) \sim E(G)} \Ind[X_u - X_v \neq X_u' - X_v'] \le \viol(X) + \viol(X').
    \]
\end{enumerate}
\end{fact}
See Fact~\ref{fact:z-vars} in the appendix for a proof (the guarantees are phrased in terms of the variables $Z_{u,s} = \Ind[X_u - X_u' = s]$.\footnote{The proof of the final claim follows from Fact~\ref{fact:z-vars} sub-claim ``Crossing edges violate an assignment'' and from noting that from the Booleanity and partition constraints, $\Ind[X_u - X_u' \neq X_v - X_v'] = \sum_{s \neq t} Z_{u,s}Z_{v,t} = \sum_{s\neq t} Z_{u,s}Z_{v,t}(Y_{(u,v)} + (1-Y_{u,v}))(Y'_{(u,v)} + (1-Y'_{u,v})) \le (1-Y_{u,v}) + (1-Y'_{u,v}$); the claim is required for the final inequality.})


Much of the work in these proofs will consist of arguing that the approximate indicator $p$ behaves like a true indicator.
We will appeal to the following facts, which are proven later in Section~\ref{sec:apx-ind}:

\begin{fact}[Approximate Markov Inequality]\label{fact:apx-markov}
Under the axioms of the lemma, $p \in P_{\beta,\nu}$ approximately obey Markov's inequality over $[0,1]$:
\[
\A_G \cup \{p \in P_{\beta,\nu}\} \cup \{0 \le x \le 1\} \,\,\vdash_{\tilde{O}(1/\nu)}\,\, p(x) \ge 1 - \frac{1-x}{1-\beta-\nu} - \nu.
\]
\end{fact}
See Fact~\ref{fact:bdd-markov} for a proof of a slightly more general statement.

\begin{fact}[Approximate Union Bound]\label{fact:apx-union}
The approximate events $p(x), p(y)$ satisfy the union bound:
\[
\{0 \le x,y \le 1\} \cup \{p \in P_{\beta,\nu}\} \,\, \vdash_{\tilde{O}(1/\nu)}  1 - p(x) p(y) \le (1-p(x))(1-p(y)).
\]
\end{fact}
See Fact~\ref{fact:apx-ub} for a proof of a slightly more general statement.

Now, we are ready to prove our claims.
\mitali{restate claim {claim:bounded}}
\begin{proof}[Proof of Claim~\ref{claim:bounded}]
By definition, $f_s(v) = \Ind[X_v - X_v' =s] \cdot p(\val_v(X))$.
From Fact~\ref{fact:ug-axioms} we have the axioms $\Ind[X_v -X_v' = s]$ and $0 \le \val_v(X) \le 1$ in degree-$4$, and from Theorem~\ref{thm:step-approx} we have the axiom that $0 \le p(x) \le 1$ in degree $\tilde{O}(1/\nu)$.
The conclusion follows as a consequence of these axioms, since for $0 \le A,B \le 1$,
$(1-A)B \ge 0$ and $(A-0)B \ge 0$.
\end{proof}

\mitali{restate claim {claim:cover}}
\begin{proof}[Proof of Claim~\ref{claim:cover}]
By the partition constraints (Fact~\ref{fact:ug-axioms}), for each $v \in V(G)$ 
\[
\sum_{s \in \Sigma} f_v(s) = p(\val_v(X)).
\]
From Fact~\ref{fact:apx-markov} we further have that
\[
p(\val_v(X)) 
\ge \left(1-\frac{\viol_v(X)}{1-\beta-\nu}-\nu\right),
\]
where $\viol_v(X) = 1 - \val_v(X)$, and the inequality is a sum-of-squares inequality of degree $\deg(p)+2$. 
Finally, we use that $\pi$ is the stationary measure to conclude that $\E_{v \sim \pi} \viol_v(X) = \viol(X)$, and the conclusion follows.
\end{proof}

\mitali{restate claim {claim:expans}}
\begin{proof}[Proof of Claim~\ref{claim:expans}]

We begin by expanding the left-hand side.
By definition of the Laplacian,
\begin{equation}
\sum_{s \in \Sigma} \langle f_s, L f_s \rangle_\pi
=  \sum_{s \in \Sigma} \E_{(u,v) \sim E(G)} \frac{1}{2} f_s(u)^2 + \frac{1}{2} f_s(v)^2 - f_s(u) f_s(v).\label{eq:lap-ex}
\end{equation}
We now apply the fact that the $\Ind(X_u - X_u' = s)$ satisfy Booleanity and partition axioms (Fact~\ref{fact:ug-axioms}) to obtain that $
\sum_{s} f_s(v)^2 = \sum_s \Ind(X_v - X_v'=s) p(\val_u(X))^2 = p(\val_u(X))^2 \le 1$, where the inequality is a sum-of-squares inequality, and also that $\sum_s f_s(u) f_s(v) = p(\val_v(X))p(\val_v(X))\Ind(X_u - X_v = X'_u - X'_v)$.
Combining these, we have the sum-of-squares inequality
\begin{equation}
(\ref{eq:lap-ex}) 
\le \E_{(u,v) \sim E(G)}\left( 1- p(\val_u(X))p(\val_v(X))\Ind[X_u - X_v = X_u' - X_v']\right)\label{eq:lap-2}
\end{equation}
Now we can add and subtract $\Ind[X_u - X_v = X_u' - X_v']$ to the right hand side and then apply the approximate union bound Fact~\ref{fact:apx-ub} to obtain
\begin{align}
(\ref{eq:lap-2}) 
&\le \E_{(u,v) \sim E(G)} \left(\Ind[X_u - X_v \neq X_u' - X_v'] + \Ind[X_u - X_v = X_u' - X_v'](1-p(\val_u(X))p(\val_v(X)))\right)\nonumber\\
&\le \E_{(u,v) \sim E(G)}\left( \Ind[X_u - X_v \neq X_u' - X_v'] + (1-p(\val_v(X))) + (1-p(\val_u(X)))\right),\label{eq:lap-3}
\end{align}
with both inequalities certifiable by $O(\deg(p))$ sum-of-squares proofs.
To bound the first term $\Ind[X_u - X_v \neq X_u' - X_v']$, we use the third claim of Fact~\ref{fact:ug-axioms}, and to bound the remaining terms we apply our approximate Markov's inequality Fact~\ref{fact:apx-markov}, concluding that
\[
(\ref{eq:lap-3}) \le \viol(X) + \viol(X') + \E_{(u,v) \sim E(G)} \left(\frac{\viol_u(X)}{1-\beta-\nu} + \frac{\viol_v(X)}{1-\beta-\nu} +2\nu\right),
\]
and finally applying the property of the stationary measure that $\E_{u \sim \pi} g(u) = \E_{(u,v) \sim E(G)} g(u)$, and that $\E_{u \sim \pi} \viol_u(X) = \viol(X)$, we obtain our conclusion.
\end{proof}

\mitali{restate claim {claim:B1}}
\begin{proof}[Proof of Claim~\ref{claim:B1}]
For any $v \in V(G)$, the Booleanity and partition constraints (Fact~\ref{fact:ug-axioms}) give us that
\begin{align*}
\sum_{s \in \Sigma} f_s(v) - f_s(v)^2
&= \sum_{s \in \Sigma} \Ind[X_v - X'_v = s]\left(p(\val_v(X)) - p(\val_v(X))^2\right)\\
&=p(\val_v(X)) - p(\val_v(X))^2
\le 1- p(\val_v(X)),
\end{align*}
where we note the final inequality is an \sos inequality by applying the axiom that $p(x) \in [0,1]$ for $x \in [0,1]$, and that $\val_v(X) \in [0,1]$.
Now applying our approximate Markov's inequality (Fact~\ref{fact:apx-markov}) and the fact that $\val_v(X) = 1-\viol_v(X)$, and finally noting that $\E_{v\sim \pi}\viol_v(X) = \viol(X)$ by definition of the stationary measure, we have our conclusion.
\end{proof}

\mitali{restate claim {claim:B2}}
\begin{proof}[Proof of Claim~\ref{claim:B2}]
We apply Cauchy-Schwarz,
\[
\sum_{s \in \Sigma} \langle f_s - f_s^{\circ 3}, Pf_s\rangle_\pi \le \frac{1}{2\eta} \sum_{s} \|Pf_s\|_{\pi,2}^2 + \frac{\eta}{2}\sum_{s} \|f_s - f_s^{\circ 3}\|_{\pi,2}^2.
\]
To bound the first term on the right-hand side, we note that $P$ is a projection matrix, and therefore we can bound the sum $\sum_{s} \|Pf_s\|_{\pi,2}^2 \le \sum_{s}\|f_s\|_{\pi,2}^2 \le 1$.
Further, the inequality is an \sos inequality since the $f_s$ satisfy approximate partition constraints and we can certify that $f_s(v)\in[0,1]$ (Fact~\ref{fact:ug-axioms} and Claim~\ref{claim:bounded}).
To bound the second term on the right-hand side, we expand,
\begin{align*}
    \sum_{s \in \Sigma} \|f_s - f_s^{\circ 3}\|_{\pi,2}^2
    &= \sum_{s \in \Sigma} \E_{u \sim \pi} (f_s(u) - f_s(u)^3)^2\\
    &= \sum_{s \in \Sigma} \E_{u \sim \pi} \Ind[X_u - X_u' = s] p(\val_u(X))^2 (1 - p(\val_u(X))^2)^2,\\
    &= \E_{u \sim \pi}p(\val_u(X))^2 (1 - p(\val_u(X))^2)^2,
\end{align*}
where we have used the Booleanity and partition constraints from Fact~\ref{fact:ug-axioms}.
The same fact ensures that we have as an \sos axiom that $\val_u(X) \in [0,1]$ and therefore $p(\val_u(X))^1(1-p(\val_u(X))^2) \le 1$, so we have as an \sos inequality of degree $O(\deg(p))$,
\begin{align*}
    \sum_{s \in \Sigma} \|f_s - f_s^{\circ 3}\|_{\pi,2}^2
    &\le 1 - \E_{u \sim \pi}p(\val_u(X))^2.
\end{align*}
Now applying Observation~\ref{obs:squaring}, we have that $p^2$ shares all of the characteristics of $P_{\beta,2\nu}$ save for the degree bound, and combining this with our approximate Markov inequality (Fact~\ref{fact:apx-ub}) we get that
\begin{align*}
    \sum_{s \in \Sigma} \|f_s - f_s^{\circ 3}\|_{\pi,2}^2
    &\le \E_{u \sim \pi}\left(\frac{\viol_u(X)}{1-\beta-2\nu} + 2\nu\right).
\end{align*}
The conclusion now follows by noting that $\E_{u \sim \pi}\viol_u(X) = \viol(X)$, and by using our bound $\nu < \frac{1}{3}(1-\beta)$ to argue that $\frac{1}{2}\cdot \frac{1}{1-\beta-2\nu} \le \frac{1}{1-\beta-\nu}$.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:structure-fs-j}]
\begin{align*}
\sum_{j = 0}^r \frac{c_j \ell^j}{\gamma} \E_{a \in [n]^j}[\sum_{s}q_{a}(F_s)(\delta(F_s^{\circ 2}|_a) - \gamma)] \geq (1 - \lambda_{r+1})(1- \gamma^{1/3}\exp(r))\sum_s \delta(F_s) - \sum_s \ip{F_s, LF_s} \\+ \frac{4}{3}\sum_s \E[(F_s^{\circ 3} - F_s)\sum_{i = 0}^r F_{s,i}] + \sum_s C\E[F_s - F_s^{\circ 4}]   
\end{align*}

\begin{align*}
\sum_{j = 0}^r \frac{c_j \ell^j}{\gamma} \E_{a \in [n]^j}[\sum_{s}q_{a}(F_s)(\delta(F_s|_a) - \gamma)] \geq (1 - \lambda_{r+1})(1- \gamma^{1/3}\exp(r))\left(1 - \frac{\viol(X)+\viol(X')}{1 - \beta - \nu} - 2\nu \right) \\ - \left(\viol(X)+\viol(X')+ \frac{2\viol(X) + 2\viol(X')}{1-\beta-\nu} + 4\nu\right) \\- \frac{4}{3}\left(\frac{1}{2\eta} + \eta \left(\frac{\viol(X)+\viol(X')}{1-\beta-\nu} + 2\nu\right) \right) 
\end{align*}

\begin{align*}
\sum_{j = 0}^r \frac{c_j \ell^j}{\gamma} \E_{a \in [n]^j}[\sum_{s}q_{a}(F_s)(\delta(F_s|_a) - \gamma)] \geq (1 - \lambda_{r+1})(1- \gamma^{1/3}\exp(r)) - \viol(X)-\viol(X') \\-(1 - \lambda_{r+1})(1- \gamma^{1/3}\exp(r))\left( \frac{\viol(X)+\viol(X')}{1 - \beta - \nu} + 2\nu \right) \\ - \left( \frac{2\viol(X) + 2\viol(X')}{1-\beta-\nu} + 4\nu\right) \\- \frac{4}{3}\left(\frac{1}{2\eta} + \eta \left(\frac{\viol(X)+\viol(X')}{1-\beta-\nu} + 2\nu\right) \right) 
\end{align*}

Choosing $\gamma^{1/3}\exp(r) = 1/2$ we get:
\begin{align*}
\sum_{j = 0}^r c_j \exp(r) \ell^j \E_{a \in [n]^j}[\sum_{s}q_{a}(F_s)(\delta(F_s|_a) - \exp(-r))] \geq \frac{1 - \lambda_{r+1}}{2} - \viol(X)-\viol(X') \\-\frac{1 - \lambda_{r+1}}{2}\left( \frac{\viol(X)+\viol(X')}{1 - \beta - \nu} + 2\nu \right) \\ - \left( \frac{2\viol(X) + 2\viol(X')}{1-\beta-\nu} + 4\nu\right) \\- \frac{4}{3}\left(\frac{1}{2\eta} + \eta \left(\frac{\viol(X)+\viol(X')}{1-\beta-\nu} + 2\nu\right) \right) 
\end{align*}

Rearranging we get,
\begin{align*}
\sum_{j = 0}^r c_j \exp(r) \ell^j \E_{a \in [n]^j}[\sum_{s}q_{a}(F_s)(\delta(F_s|_a) - \exp(-r))] \geq \frac{1 - \lambda_{r+1}}{2} - \frac{2}{3\eta} \\ - (\viol(X)+\viol(X'))\left(1+\frac{3(1-\lambda_{r+1})+ 12 +8\eta}{6(1-\beta-\nu)}\right) \\- \nu\left(5 - \lambda_{r+1} + \frac{8\eta}{3}\right).
\end{align*}
\end{proof}











\mitali{Need to decide notation and check consistency: 
\begin{itemize}
    \item UG instance $I$ or $\Psi$?
    \item Subcube for Johnson: $J|_a$ or $J_a$?
    \item Pseudo-stuff with or without ``-''?
    \item $\delta(F)$ for fractional size of $F$?
    \item $J$ for subcubes of Johnson
\end{itemize}
}


==> references.tex <==
@article{lubotzky2005explicit,
  title={Explicit constructions of Ramanujan complexes of type Ad},
  author={Lubotzky, Alexander and Samuels, Beth and Vishne, Uzi},
  journal={European Journal of Combinatorics},
  volume={26},
  number={6},
  pages={965--993},
  year={2005},
  publisher={Elsevier}
}

@inproceedings{kaufman2018construction,
  title={Construction of new local spectral high dimensional expanders},
  author={Kaufman, Tali and Oppenheim, Izhar},
  booktitle={Proceedings of the 50th Annual ACM SIGACT Symposium on Theory of Computing},
  pages={773--786},
  year={2018}
}



@inproceedings{dikstein2018boolean,
  title={Boolean function analysis on high-dimensional expanders},
  author={Dikstein, Yotam and Dinur, Irit and Filmus, Yuval and Harsha, Prahladh},
  booktitle={Approximation, Randomization, and Combinatorial Optimization. Algorithms and Techniques (APPROX/RANDOM 2018)},
  year={2018},
  organization={Schloss Dagstuhl-Leibniz-Zentrum fuer Informatik}
}


@article{BuhaiKS22,
  author    = {Rares{-}Darius Buhai and
               Pravesh K. Kothari and
               David Steurer},
  title     = {Algorithms approaching the threshold for semi-random planted clique},
  journal   = {CoRR},
  volume    = {abs/2212.05619},
  year      = {2022},
  url       = {https://doi.org/10.48550/arXiv.2212.05619},
  doi       = {10.48550/arXiv.2212.05619},
  eprinttype = {arXiv},
  eprint    = {2212.05619},
  timestamp = {Mon, 02 Jan 2023 15:09:55 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2212-05619.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{BakshiDHKKK20,
  author    = {Ainesh Bakshi and
               Ilias Diakonikolas and
               Samuel B. Hopkins and
               Daniel Kane and
               Sushrut Karmalkar and
               Pravesh K. Kothari},
  title     = {Outlier-Robust Clustering of Gaussians and Other Non-Spherical Mixtures},
  booktitle = {61st {IEEE} Annual Symposium on Foundations of Computer Science, {FOCS}
               2020, Durham, NC, USA, November 16-19, 2020},
  pages     = {149--159},
  publisher = {{IEEE}},
  year      = {2020},
}
@inproceedings{BakshiDJKKV22,
  author    = {Ainesh Bakshi and
               Ilias Diakonikolas and
               He Jia and
               Daniel M. Kane and
               Pravesh K. Kothari and
               Santosh S. Vempala},
  title     = {Robustly learning mixtures of \emph{k} arbitrary Gaussians},
  booktitle = {{STOC} '22: 54th Annual {ACM} {SIGACT} Symposium on Theory of Computing,
               Rome, Italy, June 20 - 24, 2022},
  pages     = {1234--1247},
  publisher = {{ACM}},
  year      = {2022}
}

@article{schweighofer,
  title={On the complexity of Schm{\"u}dgen's Positivstellensatz},
  author={Schweighofer, Markus},
  journal={Journal of Complexity},
  volume={20},
  number={4},
  pages={529--543},
  year={2004},
  publisher={Elsevier}
}


@inproceedings{BBKSS,
  author    = {Mitali Bafna and
               Boaz Barak and
               Pravesh K. Kothari and
               Tselil Schramm and
               David Steurer},
  title     = {Playing unique games on certified small-set expanders},
  booktitle = {{STOC} '21: 53rd Annual {ACM} {SIGACT} Symposium on Theory of Computing,
               Virtual Event, Italy, June 21-25, 2021},
  pages     = {1629--1642},
  publisher = {{ACM}},
  year      = {2021},
}

@article{trevisan2014inapproximability,
  title={Inapproximability of combinatorial optimization problems},
  author={Trevisan, Luca},
  journal={Paradigms of Combinatorial Optimization: Problems and New Approaches},
  pages={381--434},
  year={2014},
  publisher={Wiley Online Library}
}

@article{trevisan2012khot,
  title={ON KHOT'S UNIQUE GAMES CONJECTURE.},
  author={Trevisan, Luca},
  journal={Bulletin (New Series) of the American Mathematical Society},
  volume={49},
  number={1},
  year={2012},
  publisher={Citeseer}
}

@article{filmus2020hypercontractivity,
  title={Hypercontractivity on the symmetric group},
  author={Filmus, Yuval and Kindler, Guy and Lifshitz, Noam and Minzer, Dor},
  journal={arXiv preprint arXiv:2009.05503},
  year={2020}
}

@article{keevash2021global,
  title={Global hypercontractivity and its applications},
  author={Keevash, Peter and Lifshitz, Noam and Long, Eoin and Minzer, Dor},
  journal={arXiv preprint arXiv:2103.04604},
  year={2021}
}

@inproceedings{bafna2022hypercontractivity,
  title={Hypercontractivity on high dimensional expanders},
  author={Bafna, Mitali and Hopkins, Max and Kaufman, Tali and Lovett, Shachar},
  booktitle={Proceedings of the 54th Annual ACM SIGACT Symposium on Theory of Computing},
  pages={185--194},
  year={2022}
}

@inproceedings{gur2022hypercontractivity,
  title={Hypercontractivity on high dimensional expanders},
  author={Gur, Tom and Lifshitz, Noam and Liu, Siqi},
  booktitle={Proceedings of the 54th Annual ACM SIGACT Symposium on Theory of Computing},
  pages={176--184},
  year={2022}
}

@article{Raz,
  author    = {Ran Raz},
  title     = {A Parallel Repetition Theorem},
  journal   = {{SIAM} J. Comput.},
  volume    = {27},
  number    = {3},
  pages     = {763--803},
  year      = {1998},
  url       = {https://doi.org/10.1137/S0097539795280895},
  doi       = {10.1137/S0097539795280895},
  timestamp = {Wed, 14 Nov 2018 10:45:08 +0100},
  biburl    = {https://dblp.org/rec/journals/siamcomp/Raz98.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{KMMS,
  author    = {Subhash Khot and
               Dor Minzer and
               Dana Moshkovitz and
               Muli Safra},
  title     = {Small Set Expansion in The Johnson Graph},
  journal   = {Electron. Colloquium Comput. Complex.},
  volume    = {{TR18-078}},
  year      = {2018},
  url       = {https://eccc.weizmann.ac.il/report/2018/078},
  eprinttype = {ECCC},
  eprint    = {TR18-078},
  timestamp = {Tue, 27 Sep 2022 23:15:37 +0200},
  biburl    = {https://dblp.org/rec/journals/eccc/KhotMMS18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/soda/BafnaHKL22,
  author    = {Mitali Bafna and
               Max Hopkins and
               Tali Kaufman and
               Shachar Lovett},
  title     = {High Dimensional Expanders: Eigenstripping, Pseudorandomness, and
               Unique Games},
  booktitle = {Proceedings of the 2022 {ACM-SIAM} Symposium on Discrete Algorithms,
               {SODA} 2022, Virtual Conference / Alexandria, VA, USA, January 9 -
               12, 2022},
  pages     = {1069--1128},
  year      = {2022}
}

@inproceedings{DBLP:conf/stoc/DinurKKMS18a,
  author    = {Irit Dinur and
               Subhash Khot and
               Guy Kindler and
               Dor Minzer and
               Muli Safra},
  editor    = {Ilias Diakonikolas and
               David Kempe and
               Monika Henzinger},
  title     = {On non-optimally expanding sets in Grassmann graphs},
  booktitle = {Proceedings of the 50th Annual {ACM} {SIGACT} Symposium on Theory
               of Computing, {STOC} 2018, Los Angeles, CA, USA, June 25-29, 2018},
  pages     = {940--951},
  publisher = {{ACM}},
  year      = {2018},
  url       = {https://doi.org/10.1145/3188745.3188806},
  doi       = {10.1145/3188745.3188806},
  timestamp = {Wed, 21 Nov 2018 12:44:02 +0100},
  biburl    = {https://dblp.org/rec/conf/stoc/DinurKKMS18a.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{MMlocalexpander,
  author    = {Konstantin Makarychev and
               Yury Makarychev},
  editor    = {Klaus Jansen and
               Roberto Solis{-}Oba},
  title     = {How to Play Unique Games on Expanders},
  booktitle = {Approximation and Online Algorithms - 8th International Workshop,
               {WAOA} 2010, Liverpool, UK, September 9-10, 2010. Revised Papers},
  series    = {Lecture Notes in Computer Science},
  volume    = {6534},
  pages     = {190--200},
  publisher = {Springer},
  year      = {2010},
  url       = {https://doi.org/10.1007/978-3-642-18318-8\_17},
  doi       = {10.1007/978-3-642-18318-8\_17},
  timestamp = {Tue, 14 May 2019 10:00:46 +0200},
  biburl    = {https://dblp.org/rec/conf/waoa/MakarychevM10.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{KhotICM,
  author    = {Subhash Khot},
  title     = {On the Unique Games Conjecture (Invited Survey)},
  booktitle = {Proceedings of the 25th Annual {IEEE} Conference on Computational
               Complexity, {CCC} 2010, Cambridge, Massachusetts, USA, June 9-12,
               2010},
  pages     = {99--121},
  publisher = {{IEEE} Computer Society},
  year      = {2010},
  url       = {https://doi.org/10.1109/CCC.2010.19},
  doi       = {10.1109/CCC.2010.19},
  timestamp = {Tue, 21 Jul 2020 19:04:52 +0200},
  biburl    = {https://dblp.org/rec/conf/coco/Khot10.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{KNSgroth,
  author    = {Guy Kindler and
               Assaf Naor and
               Gideon Schechtman},
  title     = {The {UGC} Hardness Threshold of the \emph{L\({}_{\mbox{p}}\)} Grothendieck
               Problem},
  journal   = {Math. Oper. Res.},
  volume    = {35},
  number    = {2},
  pages     = {267--283},
  year      = {2010},
  url       = {https://doi.org/10.1287/moor.1090.0425},
  doi       = {10.1287/moor.1090.0425},
  timestamp = {Sun, 28 May 2017 13:24:38 +0200},
  biburl    = {https://dblp.org/rec/journals/mor/KindlerNS10.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Austrin,
  author    = {Per Austrin},
  editor    = {David S. Johnson and
               Uriel Feige},
  title     = {Balanced max 2-sat might not be the hardest},
  booktitle = {Proceedings of the 39th Annual {ACM} Symposium on Theory of Computing,
               San Diego, California, USA, June 11-13, 2007},
  pages     = {189--197},
  publisher = {{ACM}},
  year      = {2007},
  url       = {https://doi.org/10.1145/1250790.1250818},
  doi       = {10.1145/1250790.1250818},
  timestamp = {Wed, 14 Nov 2018 10:51:37 +0100},
  biburl    = {https://dblp.org/rec/conf/stoc/Austrin07.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}



@book{Vadhan12, 
author = {Vadhan, Salil P.}, 
title = {Pseudorandomness}, 
year = {2012}, 
isbn = {1601985940}, 
publisher = {Now Publishers Inc.}, address = {Hanover, MA, USA} }
 
@article{DBLP:journals/eccc/AroraIMS10,
  author    = {Sanjeev Arora and
               Russell Impagliazzo and
               William Matthews and
               David Steurer},
  title     = {Improved Algorithms for Unique Games via Divide and Conquer},
  journal   = {Electron. Colloquium Comput. Complex.},
  volume    = {17},
  pages     = {41},
  year      = {2010},
  url       = {http://eccc.hpi-web.de/report/2010/041},
  timestamp = {Tue, 08 Sep 2020 13:26:50 +0200},
  biburl    = {https://dblp.org/rec/journals/eccc/AroraIMS10.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{GuruswamiSinop11,
  author    = {Venkatesan Guruswami and
               Ali Kemal Sinop},
  title     = {Lasserre Hierarchy, Higher Eigenvalues, and Approximation Schemes
               for Graph Partitioning and Quadratic Integer Programming with {PSD}
               Objectives},
  booktitle = {{IEEE} 52nd Annual Symposium on Foundations of Computer Science, {FOCS}
               2011, Palm Springs, CA, USA, October 22-25, 2011},
  pages     = {482--491},
  year      = {2011},
  url       = {https://doi.org/10.1109/FOCS.2011.36},
  doi       = {10.1109/FOCS.2011.36},
  timestamp = {Fri, 19 May 2017 01:26:00 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/focs/GuruswamiS11},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{TCS-086,
url = {http://dx.doi.org/10.1561/0400000086},
year = {2019},
volume = {14},
journal = {Foundations and Trends® in Theoretical Computer Science},
title = {Semialgebraic Proofs and Efficient Algorithm Design},
doi = {10.1561/0400000086},
issn = {1551-305X},
number = {1-2},
pages = {1-221},
author = {Noah Fleming and Pravesh Kothari and Toniann Pitassi}
}
@inproceedings{DinurKKMS18,
  title={Towards a proof of the 2-to-1 games conjecture?},
  author={Dinur, Irit and Khot, Subhash and Kindler, Guy and Minzer, Dor and Safra, Muli},
  booktitle={Proceedings of the 50th Annual ACM SIGACT Symposium on Theory of Computing},
  pages={376--389},
  year={2018}
}

@inproceedings{BKS17,
  author    = {Boaz Barak and
               Pravesh K. Kothari and
               David Steurer},
  title     = {Quantum entanglement, sum of squares, and the log rank conjecture},
  booktitle = {Proceedings of the 49th Annual {ACM} {SIGACT} Symposium on Theory
               of Computing, {STOC} 2017, Montreal, QC, Canada, June 19-23, 2017},
  pages     = {975--988},
  year      = {2017},
  url       = {https://doi.org/10.1145/3055399.3055488},
  doi       = {10.1145/3055399.3055488},
  timestamp = {Sun, 02 Jun 2019 21:10:31 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/stoc/BarakKS17},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Khot02,
  author    = {Subhash Khot},
  title     = {On the power of unique 2-prover 1-round games},
  booktitle = {Proceedings on 34th Annual {ACM} Symposium on Theory of Computing,
               May 19-21, 2002, Montr{\'{e}}al, Qu{\'{e}}bec, Canada},
  pages     = {767--775},
  year      = {2002},
  url       = {https://doi.org/10.1145/509907.510017},
  doi       = {10.1145/509907.510017},
  timestamp = {Wed, 14 Nov 2018 10:51:36 +0100},
  biburl    = {https://dblp.org/rec/bib/conf/stoc/Khot02a},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@proceedings{DBLP:conf/stoc/2002,
  editor    = {John H. Reif},
  title     = {Proceedings on 34th Annual {ACM} Symposium on Theory of Computing,
               May 19-21, 2002, Montr{\'{e}}al, Qu{\'{e}}bec, Canada},
  publisher = {{ACM}},
  year      = {2002},
  isbn      = {1-58113-495-9},
  timestamp = {Thu, 16 Feb 2012 12:04:12 +0100},
  biburl    = {https://dblp.org/rec/bib/conf/stoc/2002},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{KhotMS18,
  author    = {Subhash Khot and
               Dor Minzer and
               Muli Safra},
  title     = {Pseudorandom Sets in Grassmann Graph Have Near-Perfect Expansion},
  booktitle = {59th {IEEE} Annual Symposium on Foundations of Computer Science, {FOCS}
               2018, Paris, France, October 7-9, 2018},
  pages     = {592--601},
  year      = {2018},
  url       = {https://doi.org/10.1109/FOCS.2018.00062},
  doi       = {10.1109/FOCS.2018.00062},
  timestamp = {Sun, 23 Dec 2018 08:29:07 +0100},
  biburl    = {https://dblp.org/rec/bib/conf/focs/KhotMS18},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@proceedings{DBLP:conf/focs/2018,
  editor    = {Mikkel Thorup},
  title     = {59th {IEEE} Annual Symposium on Foundations of Computer Science, {FOCS}
               2018, Paris, France, October 7-9, 2018},
  publisher = {{IEEE} Computer Society},
  year      = {2018},
  url       = {http://ieeexplore.ieee.org/xpl/mostRecentIssue.jsp?punumber=8554191},
  isbn      = {978-1-5386-4230-6},
  timestamp = {Tue, 04 Dec 2018 10:32:10 +0100},
  biburl    = {https://dblp.org/rec/bib/conf/focs/2018},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{KhotKMO07,
  author    = {Subhash Khot and
               Guy Kindler and
               Elchanan Mossel and
               Ryan O'Donnell},
  title     = {Optimal Inapproximability Results for {MAX-CUT} and Other 2-Variable
               CSPs?},
  journal   = {{SIAM} J. Comput.},
  volume    = {37},
  number    = {1},
  pages     = {319--357},
  year      = {2007},
  url       = {https://doi.org/10.1137/S0097539705447372},
  doi       = {10.1137/S0097539705447372},
  timestamp = {Wed, 14 Nov 2018 10:45:06 +0100},
  biburl    = {https://dblp.org/rec/bib/journals/siamcomp/KhotKMO07},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{Raghavendra08,
  author    = {Prasad Raghavendra},
  title     = {Optimal algorithms and inapproximability results for every CSP?},
  booktitle = {Proceedings of the 40th Annual {ACM} Symposium on Theory of Computing,
               Victoria, British Columbia, Canada, May 17-20, 2008},
  pages     = {245--254},
  year      = {2008},
  url       = {https://doi.org/10.1145/1374376.1374414},
  doi       = {10.1145/1374376.1374414},
  timestamp = {Wed, 14 Nov 2018 10:51:36 +0100},
  biburl    = {https://dblp.org/rec/bib/conf/stoc/Raghavendra08},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@proceedings{DBLP:conf/stoc/2008,
  editor    = {Cynthia Dwork},
  title     = {Proceedings of the 40th Annual {ACM} Symposium on Theory of Computing,
               Victoria, British Columbia, Canada, May 17-20, 2008},
  publisher = {{ACM}},
  year      = {2008},
  isbn      = {978-1-60558-047-0},
  timestamp = {Sat, 19 Jun 2010 14:44:24 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/stoc/2008},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{ChawlaKKRS06,
  author    = {Shuchi Chawla and
               Robert Krauthgamer and
               Ravi Kumar and
               Yuval Rabani and
               D. Sivakumar},
  title     = {On the Hardness of Approximating Multicut and Sparsest-Cut},
  journal   = {Computational Complexity},
  volume    = {15},
  number    = {2},
  pages     = {94--114},
  year      = {2006},
  url       = {https://doi.org/10.1007/s00037-006-0210-9},
  doi       = {10.1007/s00037-006-0210-9},
  timestamp = {Sun, 17 Dec 2017 22:06:00 +0100},
  biburl    = {https://dblp.org/rec/bib/journals/cc/ChawlaKKRS06},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{KhotR08,
  author    = {Subhash Khot and
               Oded Regev},
  title     = {Vertex cover might be hard to approximate to within 2-epsilon},
  journal   = {J. Comput. Syst. Sci.},
  volume    = {74},
  number    = {3},
  pages     = {335--349},
  year      = {2008},
  url       = {https://doi.org/10.1016/j.jcss.2007.06.019},
  doi       = {10.1016/j.jcss.2007.06.019},
  timestamp = {Sat, 20 May 2017 00:25:52 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/jcss/KhotR08},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/stoc/CherapanamjeriH20,
  author    = {Yeshwanth Cherapanamjeri and
               Samuel B. Hopkins and
               Tarun Kathuria and
               Prasad Raghavendra and
               Nilesh Tripuraneni},
  editor    = {Konstantin Makarychev and
               Yury Makarychev and
               Madhur Tulsiani and
               Gautam Kamath and
               Julia Chuzhoy},
  title     = {Algorithms for heavy-tailed statistics: regression, covariance estimation,
               and beyond},
  booktitle = {Proccedings of the 52nd Annual {ACM} {SIGACT} Symposium on Theory
               of Computing, {STOC} 2020, Chicago, IL, USA, June 22-26, 2020},
  pages     = {601--609},
  publisher = {{ACM}},
  year      = {2020},
  url       = {https://doi.org/10.1145/3357713.3384329},
  doi       = {10.1145/3357713.3384329},
  timestamp = {Tue, 09 Jun 2020 13:03:16 +0200},
  biburl    = {https://dblp.org/rec/conf/stoc/CherapanamjeriH20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{DBLP:journals/corr/abs-2005-06417,
  author    = {Ilias Diakonikolas and
               Samuel B. Hopkins and
               Daniel Kane and
               Sushrut Karmalkar},
  title     = {Robustly Learning any Clusterable Mixture of Gaussians},
  journal   = {CoRR},
  volume    = {abs/2005.06417},
  year      = {2020},
  url       = {https://arxiv.org/abs/2005.06417},
  archivePrefix = {arXiv},
  eprint    = {2005.06417},
  timestamp = {Thu, 14 May 2020 16:56:02 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2005-06417.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-2005-02970,
  author    = {Ainesh Bakshi and
               Pravesh Kothari},
  title     = {Outlier-Robust Clustering of Non-Spherical Mixtures},
  journal   = {CoRR},
  volume    = {abs/2005.02970},
  year      = {2020},
}

@article{DBLP:journals/corr/abs-1711-07465,
  author    = {Pravesh K. Kothari and
               Jacob Steinhardt},
  title     = {Better Agnostic Clustering Via Relaxed Tensor Norms},
  journal   = {CoRR},
  volume    = {abs/1711.07465},
  year      = {2017}
}

@article{DBLP:journals/corr/abs-1711-11581,
  author    = {Pravesh K. Kothari and
               David Steurer},
  title     = {Outlier-robust moment-estimation via sum-of-squares},
  journal   = {CoRR},
  volume    = {abs/1711.11581},
  year      = {2017},
  url       = {http://arxiv.org/abs/1711.11581},
  archivePrefix = {arXiv},
  eprint    = {1711.11581},
  timestamp = {Mon, 13 Aug 2018 16:48:59 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1711-11581.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{KhotMS17,
  author    = {Subhash Khot and
               Dor Minzer and
               Muli Safra},
  title     = {On independent sets, 2-to-2 games, and Grassmann graphs},
  booktitle = {Proceedings of the 49th Annual {ACM} {SIGACT} Symposium on Theory
               of Computing, {STOC} 2017, Montreal, QC, Canada, June 19-23, 2017},
  pages     = {576--589},
  year      = {2017},
  url       = {https://doi.org/10.1145/3055399.3055432},
  doi       = {10.1145/3055399.3055432},
  timestamp = {Sun, 02 Jun 2019 21:10:31 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/stoc/KhotMS17},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@proceedings{DBLP:conf/stoc/2018,
  editor    = {Ilias Diakonikolas and
               David Kempe and
               Monika Henzinger},
  title     = {Proceedings of the 50th Annual {ACM} {SIGACT} Symposium on Theory
               of Computing, {STOC} 2018, Los Angeles, CA, USA, June 25-29, 2018},
  publisher = {{ACM}},
  year      = {2018},
  url       = {http://dl.acm.org/citation.cfm?id=3188745},
  timestamp = {Thu, 21 Jun 2018 08:21:03 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/stoc/2018},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{BarakKS19,
  author    = {Boaz Barak and
               Pravesh K. Kothari and
               David Steurer},
  title     = {Small-Set Expansion in Shortcode Graph and the 2-to-2 Conjecture},
  booktitle = {10th Innovations in Theoretical Computer Science Conference, {ITCS}
               2019, January 10-12, 2019, San Diego, California, {USA}},
  pages     = {9:1--9:12},
  year      = {2019},
  url       = {https://doi.org/10.4230/LIPIcs.ITCS.2019.9},
  doi       = {10.4230/LIPIcs.ITCS.2019.9},
  timestamp = {Mon, 27 May 2019 15:36:31 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/innovations/BarakKS19},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@proceedings{DBLP:conf/innovations/2019,
  editor    = {Avrim Blum},
  title     = {10th Innovations in Theoretical Computer Science Conference, {ITCS}
               2019, January 10-12, 2019, San Diego, California, {USA}},
  series    = {LIPIcs},
  volume    = {124},
  publisher = {Schloss Dagstuhl - Leibniz-Zentrum fuer Informatik},
  year      = {2018},
  url       = {http://www.dagstuhl.de/dagpub/978-3-95977-095-8},
  isbn      = {978-3-95977-095-8},
  timestamp = {Mon, 27 May 2019 15:36:31 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/innovations/2019},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{AgarwalKKT15,
  author    = {Naman Agarwal and
               Guy Kindler and
               Alexandra Kolla and
               Luca Trevisan},
  title     = {Unique Games on the Hypercube},
  journal   = {Chicago J. Theor. Comput. Sci.},
  volume    = {2015},
  year      = {2015},
  url       = {http://cjtcs.cs.uchicago.edu/articles/2015/1/contents.html},
  timestamp = {Fri, 13 Mar 2015 12:47:30 +0100},
  biburl    = {https://dblp.org/rec/bib/journals/cjtcs/AgarwalKKT15},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{BarakBHKSZ12,
  author    = {Boaz Barak and
               Fernando G. S. L. Brand{\~{a}}o and
               Aram Wettroth Harrow and
               Jonathan A. Kelner and
               David Steurer and
               Yuan Zhou},
  title     = {Hypercontractivity, sum-of-squares proofs, and their applications},
  booktitle = {Proceedings of the 44th Symposium on Theory of Computing Conference,
               {STOC} 2012, New York, NY, USA, May 19 - 22, 2012},
  pages     = {307--326},
  year      = {2012},
  url       = {https://doi.org/10.1145/2213977.2214006},
  doi       = {10.1145/2213977.2214006},
  timestamp = {Sun, 02 Jun 2019 21:10:32 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/stoc/BarakBHKSZ12},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@proceedings{DBLP:conf/stoc/2012,
  editor    = {Howard J. Karloff and
               Toniann Pitassi},
  title     = {Proceedings of the 44th Symposium on Theory of Computing Conference,
               {STOC} 2012, New York, NY, USA, May 19 - 22, 2012},
  publisher = {{ACM}},
  year      = {2012},
  url       = {http://dl.acm.org/citation.cfm?id=2213977},
  isbn      = {978-1-4503-1245-5},
  timestamp = {Tue, 22 May 2012 21:36:43 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/stoc/2012},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{ODonnellZ13,
  author    = {Ryan O'Donnell and
               Yuan Zhou},
  title     = {Approximability and proof complexity},
  booktitle = {Proceedings of the Twenty-Fourth Annual {ACM-SIAM} Symposium on Discrete
               Algorithms, {SODA} 2013, New Orleans, Louisiana, USA, January 6-8,
               2013},
  pages     = {1537--1556},
  year      = {2013},
  url       = {https://doi.org/10.1137/1.9781611973105.111},
  doi       = {10.1137/1.9781611973105.111},
  timestamp = {Mon, 24 Jun 2019 09:03:37 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/soda/ODonnellZ13},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@proceedings{DBLP:conf/soda/2013,
  editor    = {Sanjeev Khanna},
  title     = {Proceedings of the Twenty-Fourth Annual {ACM-SIAM} Symposium on Discrete
               Algorithms, {SODA} 2013, New Orleans, Louisiana, USA, January 6-8,
               2013},
  publisher = {{SIAM}},
  year      = {2013},
  url       = {https://doi.org/10.1137/1.9781611973105},
  doi       = {10.1137/1.9781611973105},
  isbn      = {978-1-61197-251-1},
  timestamp = {Wed, 24 May 2017 08:31:20 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/soda/2013},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{ABS,
  author    = {Sanjeev Arora and
               Boaz Barak and
               David Steurer},
  title     = {Subexponential Algorithms for Unique Games and Related Problems},
  journal   = {J. {ACM}},
  volume    = {62},
  number    = {5},
  pages     = {42:1--42:25},
  year      = {2015},
  url       = {https://doi.org/10.1145/2775105},
  doi       = {10.1145/2775105},
  timestamp = {Wed, 14 Nov 2018 10:35:25 +0100},
  biburl    = {https://dblp.org/rec/bib/journals/jacm/AroraBS15},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@phdthesis{Steurer-thesis,
    title    = {On the complexity of Unique Games and graph expansion},
    school   = {Princeton University},
    author   = {Steurer, David},
    year     = {2011}
}
@inproceedings{RaghavendraST12,
  author    = {Prasad Raghavendra and
               David Steurer and
               Madhur Tulsiani},
  title     = {Reductions between Expansion Problems},
  booktitle = {Proceedings of the 27th Conference on Computational Complexity, {CCC}
               2012, Porto, Portugal, June 26-29, 2012},
  pages     = {64--73},
  year      = {2012},
  url       = {https://doi.org/10.1109/CCC.2012.43},
  doi       = {10.1109/CCC.2012.43},
  timestamp = {Tue, 23 May 2017 01:06:04 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/coco/RaghavendraST12},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@proceedings{DBLP:conf/coco/2012,
  title     = {Proceedings of the 27th Conference on Computational Complexity, {CCC}
               2012, Porto, Portugal, June 26-29, 2012},
  publisher = {{IEEE} Computer Society},
  year      = {2012},
  url       = {http://ieeexplore.ieee.org/xpl/mostRecentIssue.jsp?punumber=6242817},
  isbn      = {978-1-4673-1663-7},
  timestamp = {Fri, 13 May 2016 10:26:14 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/coco/2012},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{AroraKKSTV08,
  author    = {Sanjeev Arora and
               Subhash Khot and
               Alexandra Kolla and
               David Steurer and
               Madhur Tulsiani and
               Nisheeth K. Vishnoi},
  title     = {Unique games on expanding constraint graphs are easy: extended abstract},
  booktitle = {Proceedings of the 40th Annual {ACM} Symposium on Theory of Computing,
               Victoria, British Columbia, Canada, May 17-20, 2008},
  pages     = {21--28},
  year      = {2008},
  url       = {https://doi.org/10.1145/1374376.1374380},
  doi       = {10.1145/1374376.1374380},
  timestamp = {Tue, 06 Nov 2018 11:07:05 +0100},
  biburl    = {https://dblp.org/rec/bib/conf/stoc/AroraKKSTV08},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{MakarychevM10,
  author    = {Konstantin Makarychev and
               Yury Makarychev},
  title     = {How to Play Unique Games on Expanders},
  booktitle = {Approximation and Online Algorithms - 8th International Workshop,
               {WAOA} 2010, Liverpool, UK, September 9-10, 2010. Revised Papers},
  pages     = {190--200},
  year      = {2010},
  url       = {https://doi.org/10.1007/978-3-642-18318-8\_17},
  doi       = {10.1007/978-3-642-18318-8\_17},
  timestamp = {Tue, 14 May 2019 10:00:46 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/waoa/MakarychevM10},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@proceedings{DBLP:conf/waoa/2010,
  editor    = {Klaus Jansen and
               Roberto Solis{-}Oba},
  title     = {Approximation and Online Algorithms - 8th International Workshop,
               {WAOA} 2010, Liverpool, UK, September 9-10, 2010. Revised Papers},
  series    = {Lecture Notes in Computer Science},
  volume    = {6534},
  publisher = {Springer},
  year      = {2011},
  url       = {https://doi.org/10.1007/978-3-642-18318-8},
  doi       = {10.1007/978-3-642-18318-8},
  isbn      = {978-3-642-18317-1},
  timestamp = {Tue, 14 May 2019 10:00:46 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/waoa/2010},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/focs/KollaMM11,
  author    = {Alexandra Kolla and
               Konstantin Makarychev and
               Yury Makarychev},
  title     = {How to Play Unique Games Against a Semi-random Adversary: Study of
               Semi-random Models of Unique Games},
  booktitle = {{IEEE} 52nd Annual Symposium on Foundations of Computer Science, {FOCS}
               2011, Palm Springs, CA, USA, October 22-25, 2011},
  pages     = {443--452},
  year      = {2011},
  url       = {https://doi.org/10.1109/FOCS.2011.78},
  doi       = {10.1109/FOCS.2011.78},
  timestamp = {Fri, 19 May 2017 01:25:59 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/focs/KollaMM11},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@proceedings{DBLP:conf/focs/2011,
  editor    = {Rafail Ostrovsky},
  title     = {{IEEE} 52nd Annual Symposium on Foundations of Computer Science, {FOCS}
               2011, Palm Springs, CA, USA, October 22-25, 2011},
  publisher = {{IEEE} Computer Society},
  year      = {2011},
  url       = {http://ieeexplore.ieee.org/xpl/mostRecentIssue.jsp?punumber=6108120},
  isbn      = {978-1-4577-1843-4},
  timestamp = {Mon, 15 Dec 2014 18:48:45 +0100},
  biburl    = {https://dblp.org/rec/bib/conf/focs/2011},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{KollaMM11,
  author    = {Alexandra Kolla and
               Konstantin Makarychev and
               Yury Makarychev},
  title     = {How to Play Unique Games Against a Semi-random Adversary: Study of
               Semi-random Models of Unique Games},
  booktitle = {{IEEE} 52nd Annual Symposium on Foundations of Computer Science, {FOCS}
               2011, Palm Springs, CA, USA, October 22-25, 2011},
  pages     = {443--452},
  year      = {2011},
  url       = {https://doi.org/10.1109/FOCS.2011.78},
  doi       = {10.1109/FOCS.2011.78},
  timestamp = {Fri, 19 May 2017 01:25:59 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/focs/KollaMM11},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
p.org/rec/bib/conf/focs/2011},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{Kolla10,
  author    = {Alexandra Kolla},
  title     = {Spectral Algorithms for Unique Games},
  booktitle = {Proceedings of the 25th Annual {IEEE} Conference on Computational
               Complexity, {CCC} 2010, Cambridge, Massachusetts, USA, June 9-12,
               2010},
  pages     = {122--130},
  year      = {2010},
  url       = {https://doi.org/10.1109/CCC.2010.20},
  doi       = {10.1109/CCC.2010.20},
  timestamp = {Tue, 19 Jun 2018 18:38:00 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/coco/Kolla10},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@proceedings{DBLP:conf/coco/2010,
  title     = {Proceedings of the 25th Annual {IEEE} Conference on Computational
               Complexity, {CCC} 2010, Cambridge, Massachusetts, USA, June 9-12,
               2010},
  publisher = {{IEEE} Computer Society},
  year      = {2010},
  url       = {http://ieeexplore.ieee.org/xpl/mostRecentIssue.jsp?punumber=5497049},
  isbn      = {978-0-7695-4060-3},
  timestamp = {Tue, 19 Jun 2018 18:38:00 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/coco/2010},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{BarakS14,
  title={Sum-of-squares proofs and the quest toward optimal algorithms},
  author={Barak, Boaz and Steurer, David},
  journal={arXiv preprint arXiv:1404.5236},
  year={2014},
}

@inbook{RaghavendraSS18,
  title={High-dimensional estimation via sum-of-squares proofs},
  author={Raghavendra, Prasad and Schramm, Tselil and Steurer, David},
  booktitle = {Proceedings of the International Congress of Mathematicians (ICM 2018)},
  chapter = {},
  pages = {3389-3423},
  year = {2018},
  publisher = {World Scientific}
}


@phdthesis{Parrilo00,
	title = {Structured semidefinite programs and semialgebraic geometry methods in robustness and optimization},
	author = {Parrilo, Pablo A},
	year = {2000},
	school = {California Institute of Technology}
}
@article{Lasserre00,
	AUTHOR = {Lasserre, Jean B.},
	TITLE = {Global optimization with polynomials and the problem of
		moments},
	JOURNAL = {SIAM J. Optim.},
	FJOURNAL = {SIAM Journal on Optimization},
	VOLUME = {11},
	YEAR = {2000/01},
	NUMBER = {3},
	PAGES = {796--817},
	ISSN = {1052-6234},
	MRCLASS = {90C26 (90C22)},
	MRNUMBER = {1814045},
	MRREVIEWER = {Jos F. Sturm},
	DOI = {10.1137/S1052623400366802},
	URL = {http://dx.doi.org/10.1137/S1052623400366802}
}
@article{Shor87,
AUTHOR = {Shor, Naum},
TITLE = {Class of global minimum bounds of polynomial functions},
JOURNAL = {Cybernetics},
VOLUME = {23},
NUMBER = {6},
PAGES = {731-734},
YEAR = {1987}
}
@inproceedings{KhotM16,
  author    = {Subhash Khot and
               Dana Moshkovitz},
  title     = {Candidate hard unique game},
  booktitle = {Proceedings of the 48th Annual {ACM} {SIGACT} Symposium on Theory
               of Computing, {STOC} 2016, Cambridge, MA, USA, June 18-21, 2016},
  pages     = {63--76},
  year      = {2016},
  url       = {https://doi.org/10.1145/2897518.2897531},
  doi       = {10.1145/2897518.2897531},
  timestamp = {Tue, 06 Nov 2018 11:07:05 +0100},
  biburl    = {https://dblp.org/rec/bib/conf/stoc/KhotM16},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@proceedings{DBLP:conf/stoc/2016,
  editor    = {Daniel Wichs and
               Yishay Mansour},
  title     = {Proceedings of the 48th Annual {ACM} {SIGACT} Symposium on Theory
               of Computing, {STOC} 2016, Cambridge, MA, USA, June 18-21, 2016},
  publisher = {{ACM}},
  year      = {2016},
  url       = {http://dl.acm.org/citation.cfm?id=2897518},
  isbn      = {978-1-4503-4132-5},
  timestamp = {Fri, 10 Jun 2016 10:30:30 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/stoc/2016},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{BarakRS11,
  author    = {Boaz Barak and
               Prasad Raghavendra and
               David Steurer},
  title     = {Rounding Semidefinite Programming Hierarchies via Global Correlation},
  booktitle = {{IEEE} 52nd Annual Symposium on Foundations of Computer Science, {FOCS}
               2011, Palm Springs, CA, USA, October 22-25, 2011},
  pages     = {472--481},
  year      = {2011},
  url       = {https://doi.org/10.1109/FOCS.2011.95},
  doi       = {10.1109/FOCS.2011.95},
  timestamp = {Fri, 19 May 2017 01:26:00 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/focs/BarakRS11},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{LeiS17,
  author    = {Zhixian Lei and
               Yueqi Sheng},
  title     = {Sum of Square Proof for Brascamp-Lieb Type Inequality},
  journal   = {CoRR},
  volume    = {abs/1710.01458},
  year      = {2017},
  url       = {http://arxiv.org/abs/1710.01458},
  archivePrefix = {arXiv},
  eprint    = {1710.01458},
  timestamp = {Mon, 13 Aug 2018 16:47:51 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1710-01458},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{BarakKS14,
  author    = {Boaz Barak and
               Jonathan A. Kelner and
               David Steurer},
  title     = {Rounding sum-of-squares relaxations},
  booktitle = {Symposium on Theory of Computing, {STOC} 2014, New York, NY, USA,
               May 31 - June 03, 2014},
  pages     = {31--40},
  year      = {2014},
  url       = {https://doi.org/10.1145/2591796.2591886},
  doi       = {10.1145/2591796.2591886},
  timestamp = {Tue, 06 Nov 2018 11:07:05 +0100},
  biburl    = {https://dblp.org/rec/bib/conf/stoc/BarakKS14},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@proceedings{DBLP:conf/stoc/2014,
  editor    = {David B. Shmoys},
  title     = {Symposium on Theory of Computing, {STOC} 2014, New York, NY, USA,
               May 31 - June 03, 2014},
  publisher = {{ACM}},
  year      = {2014},
  url       = {http://dl.acm.org/citation.cfm?id=2591796},
  isbn      = {978-1-4503-2710-7},
  timestamp = {Wed, 29 Mar 2017 16:45:26 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/stoc/2014},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{diakonikolas2010bounded,
  title={Bounded independence fools halfspaces},
  author={Diakonikolas, Ilias and Gopalan, Parikshit and Jaiswal, Ragesh and Servedio, Rocco A and Viola, Emanuele},
  journal={SIAM Journal on Computing},
  volume={39},
  number={8},
  pages={3441--3462},
  year={2010},
  publisher={SIAM}
}
@book{szeg1939orthogonal,
  title={Orthogonal polynomials},
  author={Szeg\H{o}, G\'{a}bor},
  volume={23},
  year={1939},
  publisher={American Mathematical Society}
}

@inproceedings{RaghavendraS10,
  title={Graph expansion and the unique games conjecture},
  author={Raghavendra, Prasad and Steurer, David},
  booktitle={Proceedings of the forty-second ACM symposium on Theory of computing},
  pages={755--764},
  year={2010}
}

@book{O'Donnell-ABF,
  title={Analysis of boolean functions},
  author={O'Donnell, Ryan},
  year={2014},
  publisher={Cambridge University Press}
}
@article{BGHMRS15,
  title={Making the long code shorter},
  author={Barak, Boaz and Gopalan, Parikshit and H{\aa}stad, Johan and Meka, Raghu and Raghavendra, Prasad and Steurer, David},
  journal={SIAM Journal on Computing},
  volume={44},
  number={5},
  pages={1287--1324},
  year={2015},
  publisher={SIAM}
}
@article{AlonGHP92,
  title={Simple constructions of almost k-wise independent random variables},
  author={Alon, Noga and Goldreich, Oded and H{\aa}stad, Johan and Peralta, Ren{\'e}},
  journal={Random Structures \& Algorithms},
  volume={3},
  number={3},
  pages={289--304},
  year={1992},
  publisher={Wiley Online Library}
}
@inproceedings{KKL88,
  title={Influence of variables on Boolean functions},
  author={Kahn, Jeffry and Kalai, Gil and Linial, Nathan},
  booktitle={Annual Symposium on Foundations of Computer Science (Proceedings)},
  pages={68--80},
  year={1988},
  organization={Publ by IEEE}
}
@inproceedings{RaghavendraW17,
  title={On the Bit Complexity of Sum-of-Squares Proofs},
  author={Raghavendra, Prasad and Weitz, Benjamin},
  booktitle={44th International Colloquium on Automata, Languages, and Programming (ICALP 2017)},
  year={2017},
  organization={Schloss Dagstuhl-Leibniz-Zentrum fuer Informatik}
}
@article{KhotV15,
  title={The unique games conjecture, integrality gap for cut problems and embeddability of negative-type metrics into $\ell_1$},
  author={Khot, Subhash A and Vishnoi, Nisheeth K},
  journal={Journal of the ACM (JACM)},
  volume={62},
  number={1},
  pages={1--39},
  year={2015},
  publisher={ACM New York, NY, USA}
}

@inproceedings{RaghavendraS09,
  title={Integrality gaps for strong {SDP} relaxations of unique games},
  author={Raghavendra, Prasad and Steurer, David},
  booktitle={2009 50th Annual IEEE Symposium on Foundations of Computer Science},
  pages={575--585},
  year={2009},
  organization={IEEE}
}
@inproceedings{BhangaleK19,
  title={Ug-hardness to np-hardness by losing half},
  author={Bhangale, Amey and Khot, Subhash},
  booktitle={34th Computational Complexity Conference (CCC 2019)},
  year={2019},
  organization={Schloss Dagstuhl-Leibniz-Zentrum fuer Informatik}
}
@article{lee2014multiway,
  title={Multiway spectral partitioning and higher-order cheeger inequalities},
  author={Lee, James R and Gharan, Shayan Oveis and Trevisan, Luca},
  journal={Journal of the ACM (JACM)},
  volume={61},
  number={6},
  pages={1--30},
  year={2014},
  publisher={ACM New York, NY, USA}
}
@inproceedings{kwok2013improved,
  title={Improved Cheeger's inequality: Analysis of spectral partitioning algorithms through higher order spectral gap},
  author={Kwok, Tsz Chiu and Lau, Lap Chi and Lee, Yin Tat and Oveis Gharan, Shayan and Trevisan, Luca},
  booktitle={Proceedings of the forty-fifth annual ACM symposium on Theory of Computing},
  pages={11--20},
  year={2013}
}
@inproceedings{gharan2012approximating,
  title={Approximating the expansion profile and almost optimal local graph clustering},
  author={Gharan, Shayan Oveis and Trevisan, Luca},
  booktitle={2012 IEEE 53rd Annual Symposium on Foundations of Computer Science},
  pages={187--196},
  year={2012},
  organization={IEEE}
}
@article{andersen2016almost,
  title={Almost optimal local graph clustering using evolving sets},
  author={Andersen, Reid and Gharan, Shayan Oveis and Peres, Yuval and Trevisan, Luca},
  journal={Journal of the ACM (JACM)},
  volume={63},
  number={2},
  pages={1--31},
  year={2016},
  publisher={ACM New York, NY, USA}
}
@inproceedings{louis2012many,
  title={Many sparse cuts via higher eigenvalues},
  author={Louis, Anand and Raghavendra, Prasad and Tetali, Prasad and Vempala, Santosh},
  booktitle={Proceedings of the forty-fourth annual ACM symposium on Theory of computing},
  pages={1131--1140},
  year={2012}
}
@inproceedings{RT12,
  title={Approximating CSPs with global cardinality constraints using SDP hierarchies},
  author={Raghavendra, Prasad and Tan, Ning},
  booktitle={Proceedings of the twenty-third annual ACM-SIAM symposium on Discrete Algorithms},
  pages={373--387},
  year={2012},
  organization={SIAM}
}
@inproceedings{jain2019mean,
  title={Mean-field approximation, convex hierarchies, and the optimality of correlation rounding: a unified perspective},
  author={Jain, Vishesh and Koehler, Frederic and Risteski, Andrej},
  booktitle={Proceedings of the 51st Annual ACM SIGACT Symposium on Theory of Computing},
  pages={1226--1236},
  year={2019}
}
@inproceedings{kothari2018robust,
  title={Robust moment estimation and improved clustering via sum of squares},
  author={Kothari, Pravesh K and Steinhardt, Jacob and Steurer, David},
  booktitle={Proceedings of the 50th Annual ACM SIGACT Symposium on Theory of Computing},
  pages={1035--1046},
  year={2018}
}

@inproceedings{hopkins2018mixture,
  title={Mixture models, robustness, and sum of squares proofs},
  author={Hopkins, Samuel B and Li, Jerry},
  booktitle={Proceedings of the 50th Annual ACM SIGACT Symposium on Theory of Computing},
  pages={1021--1034},
  year={2018}
}

@inproceedings{ma2016polynomial,
  title={Polynomial-time tensor decompositions with sum-of-squares},
  author={Ma, Tengyu and Shi, Jonathan and Steurer, David},
  booktitle={2016 IEEE 57th Annual Symposium on Foundations of Computer Science (FOCS)},
  pages={438--446},
  year={2016},
  organization={IEEE}
}


==> tensoring.tex <==
\section{Structure theorems under graph tensoring}

\begin{enumerate}
\item Certifiable SSE $\otimes$ Certifiable SSE
\item Johnson $\otimes$ Certifiable SSE
\item Johnson $\otimes$ Johnson
\item Johnson $\otimes$ Johnson $\otimes$ Permutation graph of UG instance (will imply an algorithm for general UG)
\end{enumerate}

















